An Overview of Modest Models and Tools for Real Stochastic Timed Systems

We depend on the safe, reliable, and timely operation of cyber-physical systems ranging from smart grids to avionics components. Many of them involve time-dependent behaviours and are subject to randomness. Modelling languages and verification tools thus need to support these quantitative aspects. In my invited presentation at MARS 2022, I gave an introduction to quantitative verification using the Modest modelling language and the Modest Toolset, and highlighted three recent case studies with increasing demands on model expressiveness and tool capabilities: A case of power supply noise in a network-on-chip modelled as a Markov chain; a case of message routing in satellite constellations that uses Markov decision processes with distributed information; and a case of optimising an attack on Bitcoin via Markov automata model checking. This paper summarises the presentation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Clemens Dubslaff and Bas Luttik (Eds.):\\
Models for Formal Analysis of Real Systems (MARS 2022)\\
EPTCS 355, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.355.1}{10.4204/EPTCS.355.1}}
\pdfoutput=1

